Quantum mirrors of cubic planar graph Legendrians

For a certain class of Legendrian surfaces in the five-sphere, associated to cubic planar graphs, we show that the all-genus skein-valued holomorphic curve invariants of any filling are annihilated by certain explicit skein-valued operator equations.

==> docs/8f3e3b1d-584a-4d93-9e73-fa58b310ccf9 <==
{"id":"r0.6497335443826312","lines":[{"id":"n0.2904276040912238","blocks":[]},{"id":"n0.38974106976095513","blocks":[{"id":"n0.8367553781339622","text":"\\diagram","type":"composite","elements":{"de15052487620565658":{"id":"de15052487620565658","lines":[{"id":"n0.14051838154609053","blocks":[{"id":"n0.49166802405361376","text":"1"}]}],"shape":{"data":{"p":{"x":231,"y":124}},"anchor":"left-top"},"isTextMode":true},"de10069508912202285":{"id":"de10069508912202285","lines":[{"id":"n0.05865323264399003","blocks":[{"id":"n0.6811059601330046","text":"2"}]}],"shape":{"data":{"p":{"x":158,"y":32}},"anchor":"left-top"},"isTextMode":true},"de528225254155121":{"id":"de528225254155121","lines":[{"id":"n0.8319157837127549","blocks":[{"id":"n0.4036313256488048","text":"3"}]}],"shape":{"data":{"p":{"x":28,"y":74}},"anchor":"left-top"},"isTextMode":true},"de8962051705450776":{"id":"de8962051705450776","lines":[{"id":"n0.012961975196544628","blocks":[{"id":"n0.8573306534860431","text":"4"}]}],"shape":{"data":{"p":{"x":29.29194434766184,"y":215.70218305607534}},"anchor":"left-top"},"isTextMode":true},"de3315030315240226":{"id":"de3315030315240226","lines":[{"id":"n0.8316059556512679","blocks":[{"id":"n0.9362269717008176","text":"n"}]}],"shape":{"data":{"p":{"x":157.08305565233817,"y":253.29975485636012}},"anchor":"left-top"},"isTextMode":true},"de39530022753908656":{"id":"de39530022753908656","lines":[{"id":"n0.23332429503466157","blocks":[{"id":"n0.289513791520029","text":"2"}]}],"shape":{"data":{"p":{"x":301,"y":255}},"anchor":"left-top"},"isTextMode":true},"de4897585513868483":{"id":"de4897585513868483","lines":[{"id":"n0.00937799269408901","blocks":[{"id":"n0.03969711876178694","text":"3"}]}],"shape":{"data":{"p":{"x":428.48886293327286,"y":216.41920054496526}},"anchor":"left-top"},"isTextMode":true},"de01680676338796394":{"id":"de01680676338796394","lines":[{"id":"n0.1705854023044202","blocks":[{"id":"n0.546982730744382","text":"4"}]}],"shape":{"data":{"p":{"x":430,"y":78}},"anchor":"left-top"},"isTextMode":true},"de0957478688350416":{"id":"de0957478688350416","lines":[{"id":"n0.8848902933859284","blocks":[{"id":"n0.08779000726116504","text":"n"}]}],"shape":{"data":{"p":{"x":302,"y":32}},"anchor":"left-top"},"isTextMode":true},"de9525757364908715":{"id":"de9525757364908715","lines":[{"id":"n0.986326072338647","blocks":[{"id":"n0.887335714371556","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.5224307269625961","lines":[{"id":"n0.16357715562118857","blocks":[{"id":"n0.9034933620597064","text":"F"},{"id":"n0.12059048383536264","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.35588299085602615","lines":[{"id":"n0.8027113140335768","blocks":[{"id":"n0.8899645589381192","text":"+"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":85,"y":16}},"anchor":"left-top"},"isTextMode":true},"de7130286052844638":{"id":"de7130286052844638","lines":[{"id":"n0.07223898588511224","blocks":[{"id":"n0.6169683966725583","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.2920468879821413","lines":[{"id":"n0.047747994898938884","blocks":[{"id":"n0.3598100578290798","text":"F"},{"id":"n0.2588110226808077","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9354818121664251","lines":[{"id":"n0.4601340034549335","blocks":[{"id":"n0.7846246280725278","text":"-"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":370,"y":18}},"anchor":"left-top"},"isTextMode":true},"de5035645777347566":{"id":"de5035645777347566","lines":[{"id":"n0.8331070893789861","blocks":[{"id":"n0.04863898233728614","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.3552418834241289","lines":[{"id":"n0.9588334440410784","blocks":[{"id":"n0.8242303622949941","text":"p"},{"id":"n0.6107549763305957","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.8458641902152559","lines":[{"id":"n0.8778157007012328","blocks":[{"id":"n0.8504364146029108","text":"+"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":152,"y":180}},"anchor":"left-top"},"isTextMode":true},"de11874630009627063":{"id":"de11874630009627063","lines":[{"id":"n0.30732983155219906","blocks":[{"id":"n0.1468906771265851","text":"\\math-container","type":"composite","elements":{"mathValue":{"id":"n0.5370992671540721","lines":[{"id":"n0.6486936235862183","blocks":[{"id":"n0.5913164342357327","text":"p"},{"id":"n0.8569536880798607","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5320520947221632","lines":[{"id":"n0.194216722778206","blocks":[{"id":"n0.3716454043912004","text":"-"}]}]}}}]}]}},"displayMode":false,"style":{"mathModeType":"\\displaystyle"}}]}],"shape":{"data":{"p":{"x":298,"y":104}},"anchor":"left-top"},"isTextMode":true}},"connections":[],"intersections":{"id":"di8851754272962431","items":[],"style":{}},"shapes":[{"id":"dp8487991135011428","type":"regular-polygon","data":{"p1":{"x":24,"y":47},"p2":{"x":236.5,"y":259.50000000000006},"sides":5}},{"id":"da3159037176460585","data":[{"p1":{"x":143,"y":152.25},"p2":{"x":236.5,"y":153.25},"cp":{"dx":-70.5,"dy":-81.25},"cp2":{"dx":0,"dy":-10}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic","angleBy":0,"middle":"elg>","style":{"strokeColor":[208,2,27,1]}},{"id":"da5492057477315967","data":[{"p1":{"x":163.08305565233815,"y":52.20024514363993},"p2":{"x":103.5,"y":90},"cp":{"dx":-27.583055652338146,"dy":15.799754856360067},"cp2":{"dx":7,"dy":-20}},{"p1":{"x":103.5,"y":90},"p2":{"x":143,"y":152.25},"cp":{"dx":-7,"dy":20},"cp2":{"dx":-46.5,"dy":-9.25}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic","middle":"elg<","style":{"strokeColor":[208,2,27,1]}},{"id":"da0393455418067139","data":[{"p1":{"x":44.29194434766184,"y":90.79781694392474},"p2":{"x":71.5,"y":128},"cp":{"dx":26.20805565233816,"dy":1.2021830560752562},"cp2":{"dx":-10.773552152275954,"dy":-14.06741107801156}},{"p1":{"x":71.5,"y":128},"p2":{"x":143,"y":152.25},"cp":{"dx":10.773552152275954,"dy":14.06741107801156},"cp2":{"dx":-40.5,"dy":6.75}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic","middle":"elg<","style":{"strokeColor":[208,2,27,1]}},{"id":"da0881414740002947","data":[{"p1":{"x":44.29194434766184,"y":215.70218305607534},"p2":{"x":74.5,"y":163},"cp":{"dx":4.270673394668947,"dy":-26.485425899739653},"cp2":{"dx":-22.708559653223375,"dy":10.56361818377215}},{"p1":{"x":74.5,"y":163},"p2":{"x":143,"y":152.25},"cp":{"dx":22.708559653223375,"dy":-10.56361818377215},"cp2":{"dx":-47.5,"dy":28.75}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic","middle":"elg<","style":{"strokeColor":[208,2,27,1]}},{"id":"da9047418292176685","data":[{"p1":{"x":143,"y":152.25},"p2":{"x":163.08305565233817,"y":254.29975485636012},"cp":{"dx":-70.5,"dy":45.75},"cp2":{"dx":-20.583055652338174,"dy":-29.299754856360124}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic","middle":"elg>","style":{"strokeColor":[208,2,27,1]}},{"id":"dp8840618558683728","type":"rectangle","data":{"p1":{"x":68,"y":215},"p2":{"x":110.5,"y":257}},"style":{"strokeColor":[255,255,255,1],"boxShadow":{"fill":[255,255,255,1]},"fillColor":[255,255,255,1]}},{"id":"dp12575059455515925","type":"regular-polygon","data":{"p1":{"x":236.49999838172,"y":48.01854412320816},"p2":{"x":448.99999838171993,"y":260.5185441232083},"sides":5,"rotation":180.01}},{"id":"da3183224079009518","data":[{"p1":{"x":329.7915342135585,"y":154.949790619254},"p2":{"x":236.5,"y":154.25},"cp":{"dx":70.4858181261232,"dy":81.26230333365581},"cp2":{"dx":-0.0017453292431355294,"dy":9.99999984769127}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic","angleBy":0,"middle":"elg<","mAngleBy":4,"style":{"strokeColor":[208,2,27,1]}},{"id":"da5679751475462745","data":[{"p1":{"x":309.69101689081094,"y":254.996038797337},"p2":{"x":369.28066893740066,"y":217.20668372164266},"cp":{"dx":27.585812809642675,"dy":-15.794940464351527},"cp2":{"dx":-7.003490551870186,"dy":19.998777964912392}},{"p1":{"x":369.28066893740066,"y":217.20668372164266},"p2":{"x":329.7915342135585,"y":154.949790619254},"cp":{"dx":7.003490551870186,"dy":-19.998777964912392},"cp2":{"dx":46.498384862214664,"dy":9.258115640094985}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic","middle":"elg>","style":{"strokeColor":[208,2,27,1]}},{"id":"da7911404912355562","data":[{"p1":{"x":428.48886293327286,"y":216.41920054496526},"p2":{"x":401.2873007011367,"y":179.21226935399378},"cp":{"dx":-26.207845432642273,"dy":-1.2067572063585317},"cp2":{"dx":10.771096761792421,"dy":14.069291203315004}},{"p1":{"x":401.2873007011367,"y":179.21226935399378},"p2":{"x":329.7915342135585,"y":154.949790619254},"cp":{"dx":-10.771096761792421,"dy":-14.069291203315032},"cp2":{"dx":40.50117748038889,"dy":-6.742931313756941}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic","middle":"elg>","style":{"strokeColor":[208,2,27,1]}},{"id":"da8435417953883596","data":[{"p1":{"x":428.5106628575499,"y":91.51483633521694},"p2":{"x":398.2934093991803,"y":144.21174628830133},"cp":{"dx":-4.275295908456826,"dy":26.484680123227193},"cp2":{"dx":22.710403006525155,"dy":-10.559654631555844}},{"p1":{"x":398.2934093991803,"y":144.21174628830133},"p2":{"x":329.7915342135585,"y":154.949790619254},"cp":{"dx":-22.710403006525155,"dy":10.559654631555816},"cp2":{"dx":47.505017098107714,"dy":-28.7417092482076}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic","middle":"elg>","style":{"strokeColor":[208,2,27,1]}},{"id":"da5412888795679588","data":[{"p1":{"x":329.7915342135585,"y":154.949790619254},"p2":{"x":309.7262899092433,"y":52.89653216276838},"cp":{"dx":70.50798380751098,"dy":-45.737694732023584},"cp2":{"dx":20.577941566943593,"dy":29.30334683099366}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic","middle":"elg<","style":{"strokeColor":[208,2,27,1]}},{"id":"dp15232331673280153","type":"rectangle","data":{"p1":{"x":362.3061505273104,"y":50.20917303952125},"p2":{"x":404.80615052731054,"y":92.20917303952126},"rotation":180.01},"style":{"strokeColor":[255,255,255,1],"boxShadow":{"fill":[255,255,255,1]},"fillColor":[255,255,255,1]}},{"id":"da9645088095441989","data":[{"x":143,"y":152.25},{"x":232.47769441940585,"y":153.5432654632506},{"x":329.7915342135585,"y":154.949790619254}],"head":"no","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[74,144,226,1],"thickness":4},"middle":"fh<"}],"settings":{"grid":true}}]},{"id":"n0.10508699918736675","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":346,"delayRenderCache":{"av":346,"map":{}}}
